Emotional Attachment Framework for People-Oriented Software

In organizational and commercial settings, people often have clear roles and workflows against which functional and non-functional requirements can be extracted. However, in more social settings, such as platforms for enhancing social interaction, successful applications are driven more by using emotional engagement than functionality, and the drivers of user engagement are difficult to identify. A key challenge is to understand people's emotional goals so that they can be incorporated into the design. This paper proposes a novel framework called the Emotional Attachment Framework, which is based on existing models and theories of emotional attachment. Its aim is to facilitate the process of getting a deeper insight into emotional goals in software engineering. To demonstrate the framework in use, emotional goals are elicited for a software application that aims to provide help for homeless people. To measure the effectiveness and efficiency of the proposed technique in this study, a series of evaluations are undertaken: a semi-controlled experiment, a comparison analysis, and domain expert and end-user evaluation. The results indicate that the Emotional Attachment Framework has the potential to give better insight during analysis of emotional goals.

==> tables/POF.tex <==



==> tables/askizzy1.tex <==
\begin{table*}[!htbp]
\centering
\caption{Results of Implementing Pure Content Analysis in the Case Study}
\label{askizzy1}
%\resizebox{\textwidth}{!}{%
%\small
%\scriptsize
\footnotesize
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|p{0.3\textwidth}|p{0.26\textwidth}|c|c|c|c|c|c|c|c|}
\hline

\multirow{10}{*}{\textbf{No.}} & 
\multirow{10}{*}{\textbf{Emotional Concerns}} & \multirow{10}{*}{\textbf{Emotional Goals}} & 
\multirow{10}{*}{\textbf{\rotatebox[origin=c]{90}{Frequency}}}&
\multicolumn{7}{c|}{\textbf{Emotional Attachment Drivers}} \\ \cline{5-11}& 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  &
 
\textbf{\rotatebox[origin=c]{90}{Ideal Self}}& 
\textbf{\rotatebox[origin=c]{90}{Public Self}}& 
\textbf{\rotatebox[origin=c]{90}{Affiliation}}& 
\textbf{\rotatebox[origin=c]{90}{Social Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Ideological Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Physical Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Memories}}
   \\
 
 \cline{5-11} 
 
 &  &  &  & \multicolumn{7}{c|}{\textbf{Frequency of Emotional Codes}} \\ \hline
1 & Relieved & Having a sense of good feeling & 1 & 1 &  &  &  &  &  &  \\ \hline
2 & Desperate & Having a sense of motivation and hopefulness & 1 & 1 &  &  &  &  &  &  \\ \hline
3 & In chaos & Having a sense of priority & 1 &  & 1 &  & 1 &  &  &  \\ \hline
4 & Someone listened; My voice matters & Having a sense of being empathized  with and listened to & 2 &  &  & 2 & 2 &  &  &  \\ \hline
5 & Ashamed, Embarrassed & Having a sense of self-confidence & 2 & 2 &  &  & 2 &  &  &  \\ \hline
6 & Treated like a person, called by my name & Having a sense of being respected & 3 & 3 & 3 &  & 3 &  &  &  \\ \hline
7 & Shocked, Angry, In panic & Having a sense of calm & 3 & 3 &  &  & 2 &  &  &  \\ \hline 8 & Dignified, Respected, Stigmatized & Having a sense of self-respect and self-worth & 3 & 3 & 3 &  & 3 &  &  &  \\ \hline
9 & Belonging to a group, Connected, Isolated,  Lack of belonging, Lonely & \ Having a sense of connection and interaction & 5 &  &  & 5 & 5 &  &  &  \\ \hline
10 & Afraid of too much transparency, Worried about how the data is used, Worried about sharing my information,  Worried about too much  transparency in services, Worried about what might  happen with collected data & Having a sense of privacy & 5 &  &  &  & 5 & 4 &  &  \\ \hline
11 & Helpful, Supported, Having options & Having a sense of support and assistance & 5 &  &  &  & 5 &  &  &  \\ \hline
12 & Clarity, Confused,  Don't understand process or language,  Overwhelmed : too much terminology, Wary of wasting time with service, & Having a sense of receiving clear, simple and accurate information & 13 &  &  &  & 13 &  &  &  \\ \hline
\multicolumn{3}{|c|}{\textbf{Sum of Emotional Codes}} & \textbf{44} & \textbf{13} & \textbf{7} & \textbf{7} & \textbf{41} & \textbf{4} & \textbf{0} & \textbf{0} \\ \hline
\end{tabular}
% %}
\end{table*}

==> tables/clues.tex <==
\begin{table*}
\centering
%\small
\footnotesize
\caption{Themes Guideline}
\label{clues}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{lp{0.7\textwidth}}

\toprule
\textbf{Themes %\textbackslash Drivers
} & \textbf{Clue} 
\\ \midrule


\textbf{Self-expression} & Any evidence regarding a person's aspiration to have a distinct personal identity from others \\ %\cline{2-3} 
~~~$\bullet$ Ideal-Self & Any evidence regarding a person's aspiration  to have particular characteristics, skills, etc., \\ %\cline{2-3} 
~~$\bullet$ Public-Self & Any evidence regarding a person's aspiration to create a particular image from themselves in the eyes of others \\ %\cline{2-3} 
\midrule
\textbf{Affiliation} & Any evidence regarding a person's aspiration for connection, joining, associating, and involving  with others \\ %\cline{2-3} 
\midrule
\textbf{Pleasure} & Any evidence regarding a person's aspiration of having pleasure and happiness as the primary  or most aim of their life \\ % \cline{2-3} 
~~$\bullet$ Social Pleasure & Any evidence regarding a person's aspiration to have or improve their social interaction and  social status \\ %\cline{2-3} 
~~$\bullet$ Ideological Pleasure & Any evidence regarding a person's aspiration to follow their personal values, beliefs and  attitudes \\ %\cline{2-3} 
~~$\bullet$ Physical Pleasure & Any evidence regarding a person's aspiration to feel sense of realism in using technology \\
\midrule
\textbf{Memories} & Any evidence regarding a person's aspiration for constructing and maintaining a sense of the  past, happy moments in life or remind people, occasions, places etc. \\ 
 \bottomrule
\end{tabular}
% %}

\end{table*}





==> tables/compare.tex <==
\begin{table}[ht]
\centering
\small
%\footnotesize
%\scriptsize
\caption{The Comparison of the Results in Using POSE and EAF Approaches}
\label{compare}
%\end{table}
%\begin{table}
%\centering

\footnotesize
%%\scriptsize
%\caption{The Comparison of the Results in Using PCA and UEAF Approaches}
%\label{compare}
\begin{tabular}{lrr} 
\toprule
Count & POSE & EAF\\
\midrule
Emotional goals & 12 & 20 \\
Emotional statement & 44 & 117 \\ 
\midrule
Ideal self & 13 & 69 \\
Public self & 7 & 50 \\ 
Affiliation & 7 & 36 \\
Social pleasure & 41 & 101 \\
Ideological pleasure & 4 & 10 \\
Physical pleasure & 0 & 0 \\
Memories & 0 & 0 \\ \midrule
Self-expression & 20 & 119 \\
Affiliation & 7 & 36 \\
Memories & 0 & 0 \\
Pleasure & 45 & 111 \\
 \bottomrule
\end{tabular}
\end{table}


==> tables/negativetopositive.tex <==
\begin{table*}[!h]
\centering
%\scriptsize
%\footnotesize
\caption{Some samples of converting negative emotional concerns  to positive emotional goals}
\label{negativetopositive}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|}
\hline
\textbf{Emotional Concerns} & \textbf{Emotional Goals} \\ \hline
having cloudy mind & Having a sense of good feeling \\ \hline
Lack of People's Trust on me & Having a sense of being trusted \\ \hline
Lack of People's Respect on me & Having a sense of being respected \\ \hline
personal stress and anxiety & Having a sense of calm \\ \hline
Lack of  clarity and stability & Having a sense of receiving clear, simple and accurate information \\ \hline
People's reluctance  for support and assistance & Having a sense of support and assistance \\ \hline
Lack of privacy & Having a sense of privacy \\ \hline
Having a sense of misleading & Having a sense of receiving clear and accurate information \\ \hline
Hopelessness & Having a sense of motivation and hopefulness \\ \hline
Having a sense of misleading & Having a sense of receiving clear and accurate information \\ \hline
losing self esteem & Having a sense of self-respect and self-worth \\ \hline
Lake of empathy & Having a s sense of being empathized with and listened to. \\ \hline
Hopelessness & Having a sense of motivation and hopefulness \\ \hline
\end{tabular}%
}
\end{table*}


==> tables/oldtables.tex <==
\begin{table}[H]
\small
\centering
\caption{Goal-Driver Profile for `Sense of being in Control'}
\label{gdpSIC}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Having a Sense of In Control}}\\ Total Emotional Concerns: 1
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 100 \\
Public Self & 0 \\
Affiliation & 0 \\
Social Pleasure & 0 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}

\begin{table}[H]
\small
\centering
\caption{Goal-Driver Profile for `Sense of Empowered'}
\label{gdpSOE}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Having a Sense of Empowered}}\\ Total Emotional Concerns: 3
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 100 \\
Public Self & 0 \\
Affiliation & 0 \\
Social Pleasure & 67 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\small
\centering
\caption{Goal-Driver Profile for `Sense of Connected'}
\label{gdpSOC}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Sense of Connected}}\\ Total Emotional Concerns: 13
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 100 \\
Public Self & 100 \\
Affiliation & 92 \\
Social Pleasure & 100 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\small
\centering
\caption{Goal-Driver Profile for `Clarity and Trust of Information'}
\label{gdpSOCT}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Sense of Clarity and Trust}}\\ Total Emotional Concerns: 15
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 0 \\
Public Self & 0 \\
Affiliation & 40 \\
Social Pleasure & 100 \\
Ideological Pleasure & 0 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}


\begin{table}[!h]
\small
\centering
\caption{Goal-Driver Profile for `Sense of Self-Worth'}
\label{gdpSOS}
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}Emotional Goal: \emph{\textbf{Sense of Self-worth}}\\ Total Emotional Concerns: 5
\end{tabular}} \\ \midrule
Driver & Concerns (\%) \\ \midrule
Ideal Self & 60 \\
Public Self & 100 \\
Affiliation & 0 \\
Social Pleasure & 20 \\
Ideological Pleasure & 100 \\
Physical Pleasure & 0 \\
Memories & 0 \\ 
\hline
\end{tabular}
\end{table}

==> tables/qualitative.tex <==
\begin{table}[!t]
\centering

%\small
\caption{Qualitative Questions}
\label{tab:qualitative}
\footnotesize
\begin{tabular}{p{1.75cm}p{2cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}}
\hline

\multicolumn{1}{c}{\multirow{2}{*}{Property}} & \multicolumn{1}{c}{\multirow{2}{*}{Indices}} & \multicolumn{5}{c}{Distribution} \\ \cline{3-7} 
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & $--$ & $-$ & $\circ$ & $+$ & $++$ 

\\ \hline

 \multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Usability \&\\  Usefulness\end{tabular}} & Consistency &  &  &  & 1 &  \\  
 & Completeness &  &  &  & 1 &  \\  
 & Correctness &  &  &  & 1 &  \\ 
 & Tracability &  &  &  & 1 &  \\ 
 & Clarity &  &  &  &  & 1 \\  
 & \begin{tabular}[c]{@{}l@{}}Share \\ Understanding\end{tabular} &  &  & 1 &  &  
 
 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}} Output \\ Validity \end{tabular}} & Consistency &  &  &  &  & 1 \\  
 & Completeness &  &  &  & 1 &  \\ 
 & Correctness &  &  &  &  & 1 \\ \hline
 
\end{tabular}
\end{table}


==> tables/questions.tex <==
\begin{table*}[]
\centering
\caption{The related question for each emotional attachment driver}
\label{questions}
%\scriptsize
%\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|l|}
\hline
\textbf{Driver} & \textbf{Question} \\ \hline
Ideal Self & How this system can help me to become a person I would like to be in terms of ...  \\ \hline
Public Self & How this system can help me to create the image that  I would like other people \\ 
& have of me in terms of `a person with / who ...'  \\ \hline
Affiliation  & How this system can help me to belong to a group? \\ \hline
Social Pleasure & How this system can help me to improve my social pleasure in terms of `better social\\ 
& interaction,  better social status ...' \\ \hline
Ideological Pleasure & To what extent this system is aligned with  / respects / considers my values and \\ 
& beliefs in terms of ...  \\ \hline
Physical Pleasure & How this system can help me to feel sense of   realism in terms of ... (Sight, Hearing, Taste,  \\ & Smell 
 and Touch)"   \\ \hline
Memories & How this system can help me to remind positive memories
in terms of `something  on the \\ 
& past,  specific occasion, person, nostalgia ,...'  \\ \hline
\end{tabular}%
}
\rachel{This table is a key part of the process you undertook when extending desmets model. I would put this in the same text where you explain what each driver is. It acts as a description of how each emotional concern translates into a technology setting.}
\end{table*}


==> tables/sum1.tex <==
\begin{table}
    \centering
    \caption{Summary of emotional themes - POSE approach }
\label{sum1}
%\small
%\footnotesize

\begin{tabular}{lrrrrrrrr} 

\toprule
\textbf{} & 
\textbf{\rotatebox[origin=c]{90}{Ideal Self}}& 
\textbf{\rotatebox[origin=c]{90}{Public Self}}& 
\textbf{\rotatebox[origin=c]{90}{Affiliation}}& 
\textbf{\rotatebox[origin=c]{90}{Social Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Ideological Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Physical Pleasure}}&
\textbf{\rotatebox[origin=c]{90}{Memories}}
& \textbf{Sum}\\
\midrule
\textbf{Self-expression} & 13 & 7 &  &  &  &  &  & \textbf{20} \\
\textbf{Affiliation} &  &  & 7 &  &  &  &  & \textbf{7} \\ 
\textbf{Memories} &  &  &  &  &  &  & 0 & \textbf{0} \\
\textbf{Pleasure} &  &  &  & 41 & 4 & 0 &  & \textbf{45}\\

\bottomrule
\end{tabular}
\end{table}

